ICPL: Few-shot In-context Preference Learning via LLMs

Preference-based reinforcement learning is an effective way to handle tasks where rewards are hard to specify but can be exceedingly inefficient as preference learning is often tabula rasa. We demonstrate that Large Language Models (LLMs) have native preference-learning capabilities that allow them to achieve sample-efficient preference learning, addressing this challenge. We propose In-Context Preference Learning (ICPL), which uses in-context learning capabilities of LLMs to reduce human query inefficiency. ICPL uses the task description and basic environment code to create sets of reward functions which are iteratively refined by placing human feedback over videos of the resultant policies into the context of an LLM and then requesting better rewards. We first demonstrate ICPL's effectiveness through a synthetic preference study, providing quantitative evidence that it significantly outperforms baseline preference-based methods with much higher performance and orders of magnitude greater efficiency. We observe that these improvements are not solely coming from LLM grounding in the task but that the quality of the rewards improves over time, indicating preference learning capabilities. Additionally, we perform a series of real human preference-learning trials and observe that ICPL extends beyond synthetic settings and can work effectively with humans-in-the-loop.

==> tables/algo.tex <==
% \begin{algorithm}[htbp]
% \SetAlgoLined
% \SetKwFunction{History}{History} 
% \SetKwFunction{Feedback}{Feedback} 
% \SetKwProg{Fn}{Function}{:}{}
% \KwIn{\# iterations $N$, \# samples in each iterations $K$, environment $\texttt{Env}$, coding LLM $\texttt{LLM}_{RF}$}

% %\tcp{Use environment as context to initialize prompt}
% \tcp{Initialize the prompt containing the environment context and task description}
% $\texttt{Prompt} \gets \texttt{InitializePrompt}$

% \For{$i \gets 1$ to $N$}{
%     $\texttt{RF}_1, \dots, \texttt{RF}_K\gets \texttt{LLM}_{RF}(\texttt{Prompt}, K)$
    
%     \tcp{Render videos}
%     $\texttt{Video}_1, \dots, \texttt{Video}_K\gets \texttt{Render}(\texttt{Env}, \texttt{RF}_1), \dots, \texttt{Render}(\texttt{Env}, \texttt{RF}_K)$
    
%     \tcp{Human select the best and worst videos}
%     $G, B \gets \texttt{Human}(\texttt{Video}_1, \dots, \texttt{Video}_K)$
    
%     $\texttt{GoodRF}, \texttt{BadRF} \gets \texttt{RF}_{G}, \texttt{RF}_{B}$

%     $\texttt{Prompt} \gets \texttt{GoodRF} + \texttt{BadRF} + 
%     \texttt{HistoricalDifference} + \texttt{RewardTrace}$
% }
% \caption{\name}
% \label{Alg}
% \end{algorithm}



\begin{algorithm}[H]
    \SetAlgoLined
    \SetKwFunction{History}{History} 
    \SetKwFunction{Feedback}{Feedback} 
    \SetKwProg{Fn}{Function}{:}{}
    \KwIn{Number of iterations $N$, Number of samples $K$, Environment $\texttt{Env}$, Coding LLM $\texttt{LLM}_{RF}$}

    \tcp{Initialize the prompt with environment context and task description}
    $\texttt{Prompt} \gets \texttt{InitializePrompt}(\texttt{Env})$

    \For{$i \gets 1$ \textbf{to} $N$}{
        $\texttt{RF}_1, \dots, \texttt{RF}_K \gets \texttt{LLM}_{RF}(\texttt{Prompt}, K)$
        
        \tcp{Render videos for each reward function}
        $\texttt{Video}_1, \dots, \texttt{Video}_K \gets \texttt{Render}(\texttt{Env}, \texttt{RF}_1), \dots, \texttt{Render}(\texttt{Env}, \texttt{RF}_K)$
        
        \tcp{Human selects the most preferred (G) and least preferred (B) videos}
        $G, B \gets \texttt{Human}(\texttt{Video}_1, \dots, \texttt{Video}_K)$
        
        \tcp{Retrieve the best and worst reward functions}
        $\texttt{GoodRF}, \texttt{BadRF} \gets \texttt{RF}_G, \texttt{RF}_B$
        
        \tcp{Update the prompt with feedback}
        $\texttt{Prompt} \gets \texttt{GoodRF} + \texttt{BadRF} + \texttt{HistoricalDifference} + \texttt{RewardTrace}$
    }
    \caption{{\fullname} ({\name})}
    \label{algo: icpl}
    \end{algorithm}


==> tables/llm_choice.tex <==
\begin{table}
\centering
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{cccccccc} 
\toprule
             & Cart.                    & Ball.                                    & Ant                  & Human.               & Franka                & Shadow                & Allegro                 \\ 
\midrule
% PrefPPO-49   & {\textbf{499}{(0)}} & {\textbf{499}{(0)}}           & 0.743(0.20)          & 0.457(0.09)          & 0.0044(0.00)          & 0.0746(0.02)          & 0.0125(0.003)           \\
% PEBBLE-49  & \textbf{499}{(0)}      & \textbf{499}{(0)}           & 5.9891(2.47)  & 3.67(1.32)    & 0.0453(0.01) & 0.2627(0.03) & 0.1467(0.03)   \\
% SURF-49  & \textbf{499}{(0)}      & \textbf{499}{(0)}           & 0.874(0.18)  & 2.406(0.53)    & 0.0345(0.01) & 0.2338(0.03) & 0.2002(0.03)   \\
% PrefPPO-1.5k & {\textbf{499}{(0)}} & {\textbf{499}{(0)}}          & 4.458(1.30)          & 1.329(0.33)          & 0.3248(0.12)          & 0.0488(0.01)          & 0.0284(0.005)           \\
% PEBBLE-1.5k  & \textbf{499}{(0)}      & \textbf{499}{(0)}          & 9.364(0.71)  & 4.075(0.44)    & 0.1966(0.07) & 0.2538(0.03) & 0.2664(0.07)   \\
% SURF-1.5k  & \textbf{499}{(0)}      & \textbf{499}{(0)}         & 7.921(1.93)  & 3.577(0.24)    & 0.8032(0.27) & 0.2575(0.02) & 0.2283(0.05)   \\
%Eureka       & {\textbf{499}(0)}          & {\textbf{499}{(0)}} & 10.86(0.85)          & 9.059(0.83)          & {0.9999(0.23)} & 11.532(1.38)          & {25.250(9.583)}  \\
ICPL       & {\textbf{499}{(0)}} & {\textbf{499}{(0)}}           & {\textbf{12.04}(1.69)} & {\textbf{9.227}(0.93)} & {\textbf{0.9999}(0.24)} & {\textbf{13.231}(1.88)} & \textbf{25.030}(3.721)           \\
ICPL-GPT3.5       & {\textbf{499}{(0)}} & {\textbf{499}{(0)}}          & {10.34(3.94)} & {7.128(1.07)} & {0.0362(0.02)} & {10.084(4.13)} & 22.194(10.74)           \\
\bottomrule
\end{tabular}
}
\caption{\rebuttal{Ablation studies on the choice of LLM. The values in parentheses represent the standard deviation.}}
\label{tab: llm-choice}
\end{table}




==> tables/main.tex <==
\begin{table}
\vspace{-4mm}
\caption{The final task score of all methods across different tasks in IssacGym.
The top result and those within one standard deviation are highlighted in bold. Standard deviations are provided in Table \ref{tab: app-proxy} of Appendix \ref{app: add} due to space limitations.}
\centering
\vspace{-2mm}

\resizebox{1.0\textwidth}{!}{
\begin{tabular}{cccccccccc}
\toprule
             & Cart. & Ball. & Quad. & Anymal  & Ant    & Human. & Franka & Shadow & Allegro  \\
\midrule
PrefPPO-49   & \textbf{499}      & \textbf{499}         & -1.066     & -1.861  & 0.743  & 0.457    & 0.0044 & 0.0746 & 0.0125   \\
PrefPPO-150  & \textbf{499}      & \textbf{499}         & -0.959     & -1.818  & 0.171  & 0.607    & 0.0179 & 0.0617 & 0.0153   \\
PrefPPO-1.5k & \textbf{499}      & \textbf{499}         & -0.486     & -1.417  & 4.458  & 1.329    & 0.3248 & 0.0488 & 0.0284   \\
P
refPPO-15k  & \textbf{499}      & \textbf{499}         & -0.250     & -1.357  & 4.626  & 1.317    & 0.0399 & 0.0468 & 0.0157   \\

{\name}(Ours)   & \textbf{499}      & \textbf{499}         & \textbf{-0.0195}    & \textbf{-0.007} & \textbf{12.04} & \textbf{9.227}    & \textbf{0.9999} & \textbf{13.231} & \textbf{25.030}  \\
\hline
\hline
\rebuttal{Eureka}       & 499     & 499         & -0.023     & -0.003 & 10.86 & 9.059    & 0.9999 & 11.532 & 25.250   \\
\bottomrule
\end{tabular}
}

\label{tab: proxy}
\vspace{-3mm}
\end{table}
